Experimental Validation of Collision-Radiation Dataset for Molecular Hydrogen in Plasmas

Quantitative spectroscopy of molecular hydrogen has generated substantial demand, leading to the accumulation of diverse elementary-process data encompassing radiative transitions, electron-impact transitions, predissociations, and quenching. However, their rates currently available are still sparse and there are inconsistencies among those proposed by different authors. In this study, we demonstrate an experimental validation of such molecular dataset by composing a collisional-radiative model (CRM) for molecular hydrogen and comparing experimentally-obtained vibronic populations across multiple levels. From the population kinetics of molecular hydrogen, the importance of each elementary process in various parameter space is studied. In low-density plasmas (electron density $n_\mathrm{e} \lesssim 10^{17}\;\mathrm{m^{-3}}$) the excitation rates from the ground states and radiative decay rates, both of which have been reported previously, determines the excited state population. The inconsistency in the excitation rates affects the population distribution the most significantly in this parameter space. On the other hand, in higher density plasmas ($n_\mathrm{e} \gtrsim 10^{18}\;\mathrm{m^{-3}}$), the excitation rates \textit{from} excited states become important, which have never been reported in the literature, and may need to be approximated in some way. In order to validate these molecular datasets and approximated rates, we carried out experimental observations for two different hydrogen plasmas; a low-density radio-frequency (RF) heated plasma ($n_\mathrm{e}\approx 10^{16}\;\mathrm{m^{-3}}$) and the Large Helical Device (LHD) divertor plasma ($n_\mathrm{e}\gtrsim 10^{18}\;\mathrm{m^{-3}}$)... [continued]

==> latexmkrc <==
#!/usr/bin/perl
$latex         = 'pdflatex %O -src-specials -shell-escape -interaction=nonstopmode -synctex=1 main';
$bibtex        = 'pbibtex %O %B';
$dvipdf        = 'dvipdfmx %O -o %D main_supplemental';
$pdf_mode      = 3; # use dvipdfmx

# Use SumatraPDF and atom inverse search
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

# if you do not need to preview in -pvc option (preview document and countinuously update mode)
# $pdf_previewer = 'exit';

